Dimension theory of group actions by circle diffeomorphisms II: Minimal sets

We establish a dimension theory for smooth group actions on the circle. For finitely generated groups of real-analytic circle diffeomorphisms preserving a Cantor minimal set, we introduce a dynamically defined critical exponent and prove the following properties of that set: (1) The box dimension exists and coincides with its Hausdorff dimension; (2) The dimension is given by a formula involving the dynamical critical exponent; (3) The dimension lies strictly between $0$ and $1$; (4) A parabolic fixed point in this Cantor minimal set yields a stronger lower bound for its dimension. These results substantially generalize the classical dimension theory of limit sets of Fuchsian groups to a broader smooth setting. Moreover, item (3) strengthens a recent breakthrough of Deroin--Kleptsyn--Navas, who showed that such sets have zero Lebesgue measure. A key novelty of this work is the use of the dynamical critical exponent to link the group action with stationary and conformal measures. This provides a framework combining methods from nonuniform hyperbolic dynamics and Patterson-Sullivan theory.

==> macros.tex <==
\RequirePackage{extarrows}
\RequirePackage{bm}
\RequirePackage{mathtools}
\RequirePackage{textcomp}
\RequirePackage{wasysym}
\RequirePackage{tikz}
\RequirePackage{bbm}
\RequirePackage{graphicx}
\RequirePackage{yhmath}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage{esint}

\newcommand{\highlight}[1]{{\color{magenta} #1}}
\newcommand{\significant}[1]{\textbf{\color{red} #1}}

\DeclareMathOperator{\Dir}{\mathrm{Dirac}}

\newcommand{\Ax}{\mathrm{Ax}}
\newcommand{\leng}{\mathrm{len}}
% General
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand\LHS{\mathrm{LHS}}
\newcommand\RHS{\mathrm{RHS}}
\newcommand\cd{\, \bm\cdot\, }
\newcommand\defeq{\coloneqq}

\numberwithin{equation}{section}
\newcommand{\case}[1]{\left\{\begin{aligned}
#1
\end{aligned}\right.}
\newcommand{\lb}[1]{\left\{#1\right\}}
\newcommand{\mb}[1]{\left[#1\right]}
\renewcommand{\sb}[1]{\left(#1 \right)}
\newcommand{\msb}[1]{\left[#1\right)}
\newcommand{\smb}[1]{\left(#1 \right]}


% Abbreviation
\newcommand{\vp}{\varphi}
\newcommand{\ve}{\varepsilon}
\newcommand{\vk}{\varkappa}
\newcommand{\vn}{\varnothing}
\newcommand{\sbs}{\subset}
\newcommand{\sbse}{\subseteq}
\newcommand{\sps}{\supset}
\newcommand{\spse}{\supseteq}
\newcommand{\sm}{\setminus}
\newcommand{\ag}[1]{\begin{aligned}#1\end{aligned}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}


% Analysis
\DeclareMathOperator{\Ran}{\mathrm{Range}}
\DeclareMathOperator{\supp}{\mathrm{supp}}
\DeclareMathOperator{\Rl}{\mathrm{Re}}
\DeclareMathOperator{\Img}{\mathrm{Im}}
\DeclareMathOperator{\Lip}{\mathrm{Lip}}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\pv}{p.v.}
\DeclareMathOperator{\Spec}{\mathrm{Spec}}
\renewcommand{\ae}[1][]{\ #1\mathrm{a.e.}\ }
\newcommand{\one}{\bm{\mathbbm 1}}
\newcommand\D{\mathrm D}
\newcommand\dr{\mathrm{d}}
\newcommand{\Leb}{\mathrm{Leb}}
\newcommand{\pa}{\partial^\alpha}

\newcommand{\nm}[1]{\left\|#1\right\|}
\newcommand{\gnm}[1]{\recbracket#1\recbracket}
\newcommand{\dv}[2][0]{\left.\frac{\dr}{\dr #2}\right|_{#2=#1}}
\newcommand{\pt}[2][]{\frac{\partial#1}{\partial #2}}%partial
\newcommand{\tv}[2]{\left. #1\right|_{#2}}%take values


\newcommand{\lto}[1]{\stackrel{#1}{\longrightarrow}}
\newcommand{\pair}[1]{\left\langle#1\right\rangle}
\newcommand{\abs}[1]{\left|#1\right|}

% Dynamics
\DeclareMathOperator{\Prob}{\mathrm{Prob}}
\newcommand{\Diff}{\mathrm{Diff}}
\newcommand{\Homeo}{\mathrm{Homeo}}
\newcommand{\gr}{\mathrm{gr}}
\newcommand{\Orb}{\mathrm{Orb}}
\newcommand{\reg}{\mathrm{reg}}

% Probability
\DeclareMathOperator{\var}{var}
\renewcommand{\P}{\bm{\mathrm P}}

% Algebra
\DeclareMathOperator{\spaned}{\mathrm{span}}
\DeclareMathOperator{\Tr}{\mathrm{tr}}
\DeclareMathOperator{\rank}{\mathrm{rank}}
\renewcommand{\mod}{\ \mathrm{mod}\ }
\newcommand{\Ad}{\mathrm{Ad}}
\newcommand{\ad}{\mathrm{ad}}
\newcommand\lcm{\mathrm{lcm}}
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\End}{\mathrm{End}}
\newcommand{\Id}{\mathrm{id}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Isom}{\mathrm{Isom}}

\newcommand{\GL}{\mathrm{GL}}
\newcommand{\SL}{\mathrm{SL}}
\newcommand{\PSL}{\mathrm{PSL}}
\newcommand{\SO}{\mathrm{SO}}

\newcommand{\mtx}[1]{\footnotesize{\mb{\setlength{\arraycolsep}{2.5pt}\begin{matrix}#1\end{matrix}}}}

% Geometry
\DeclareMathOperator{\Ind}{\mathrm{Ind}}
\newcommand{\Vol}{\mathrm{Vol}}
\DeclareMathOperator{\diam}{\mathrm{diam}}



% \mathcal
\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\cH}{\mathcal H}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

% \mathscr
\newcommand{\sA}{\mathscr A}
\newcommand{\sB}{\mathscr B}
\newcommand{\sC}{\mathscr C}
\newcommand{\sD}{\mathscr D}
\newcommand{\sE}{\mathscr E}
\newcommand{\sF}{\mathscr F}
\newcommand{\sG}{\mathscr G}
\newcommand{\sH}{\mathscr H}
\newcommand{\sI}{\mathscr I}
\newcommand{\sJ}{\mathscr J}
\newcommand{\sK}{\mathscr K}
\newcommand{\sL}{\mathscr L}
\newcommand{\sM}{\mathscr N}
\newcommand{\sN}{\mathscr N}
\newcommand{\sO}{\mathscr O}
\newcommand{\sP}{\mathscr P}
\newcommand{\sQ}{\mathscr Q}
\newcommand{\sR}{\mathscr R}
\newcommand{\sS}{\mathscr S}
\newcommand{\sT}{\mathscr T}
\newcommand{\sU}{\mathscr U}
\newcommand{\sV}{\mathscr V}
\newcommand{\sW}{\mathscr W}
\newcommand{\sX}{\mathscr X}
\newcommand{\sY}{\mathscr Y}
\newcommand{\sZ}{\mathscr Z}



% \mathbb
\renewcommand{\AA}{{\mathbb A}}
\newcommand{\BB}{{\mathbb B}}
\newcommand{\CC}{{\mathbb C}}
\newcommand{\DD}{{\mathbb D}}
\newcommand{\EE}{{\mathbb E}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\II}{{\mathbb I}}
\newcommand{\JJ}{{\mathbb J}}
\newcommand{\KK}{{\mathbb K}}
\newcommand{\LL}{{\mathbb L}}
\newcommand{\MM}{{\mathbb M}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\OO}{{\mathbb O}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\RR}{{\mathbb R}}
\renewcommand{\SS}{{\mathbb S}}
\newcommand{\TT}{{\mathbb T}}
\newcommand{\UU}{{\mathbb U}}
\newcommand{\VV}{{\mathbb V}}
\newcommand{\WW}{{\mathbb W}}
\newcommand{\XX}{{\mathbb X}}
\newcommand{\YY}{{\mathbb Y}}
\newcommand{\ZZ}{{\mathbb Z}}


% \mathfrak
\newcommand{\fh}{\mathfrak h}
\newcommand{\fg}{\mathfrak g}
\newcommand{\fu}{\mathfrak u}
\newcommand{\fo}{\mathfrak o}
\newcommand{\fr}{\mathfrak r}
\newcommand{\fsu}{\mathfrak{su}}
\newcommand{\fgl}{\mathfrak{gl}}
\newcommand{\fsl}{\mathfrak{sl}}
\newcommand{\fsp}{\mathfrak{sp}}
\newcommand{\fso}{\mathfrak{so}}
\newcommand{\ft}{\mathfrak t}
\newcommand{\fz}{\mathfrak z}
\newcommand{\fs}{\mathfrak s}
\newcommand{\fM}{\mathfrak M}





\newcommand{\recbracket}{
\,
\begin{tikzpicture}[baseline]
\draw (0,-0.2em) -- (0em,0.8em) -- (0.2em,0.8em) -- (0.2em,-0.2em) -- (-0.02em,-0.2em);
\end{tikzpicture}
\,
}
\newcommand{\act}{
\,
\tikzset{every picture/.style={line width=0.07em}}
\begin{tikzpicture}[baseline]
\draw  (0,0) .. controls (0,0.8em) and (0.5em,0.8em) .. (0.5em,0);
\draw  (0.65em,0.15em) .. controls (0.56em,0.1em) and (0.52em,0.05em) .. (0.5em,0) .. controls (0.48em,0.05em) and (0.44em,0.1em) .. (0.35em,0.15em);
\end{tikzpicture}
\,
}

% WH use
\newcommand{\dd}{\,\mathrm{d}}
\newcommand{\hFur}{h_\mathrm{F}}   % Furstenberg entropy
\newcommand{\hRW}{h_\mathrm{RW}}   % Random walk entropy
\newcommand{\dimH}{\dim_\mathrm{H}}% Hausdorff dimension
\newcommand{\unif}{u}     % uniform measure
\newcommand{\Zmodd}{[d]}           % Z mod d Z
\newcommand{\CCs}{\pi_0}             % Connected components
\newcommand{\len}[1]{\lvert#1\rvert}
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\st}{st}      % cancellation
\DeclareMathOperator{\cl}{cl}      % cancellation
\DeclareMathOperator{\lcp}{lcp}      % longest common prefix
\DeclareMathOperator{\NE}{NE}
\DeclareMathOperator{\Acc}{Acc}

\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}

\DeclareMathOperator{\Nbd}{Nbd}














==> preamble.tex <==
\pagestyle{myheadings}
\RequirePackage[a4paper]{geometry}
\geometry{
  textwidth=138mm,
  textheight=215mm,
  left=27mm, 
  right=27mm, 
  top=25.4mm, 
  bottom=25.4mm,
  headheight=2.17cm,
  headsep=7mm,
  footskip=12mm,
  heightrounded,
  marginparwidth = 32mm, 
}



\markboth{{Dimension theory on circle diffeomorphisms}}
{{W.~He, Y.~Jiao, D.~Xu}}

\usepackage{amsmath, amsthm, amsfonts, amssymb}
\usepackage{epsfig, enumerate}
\usepackage{color}
\usepackage{comment}
\usepackage{hyperref}
\hypersetup{colorlinks=true,linkcolor=blue,citecolor=magenta}
\usepackage[all]{xy}
\usepackage{float}
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,trees,arrows.meta,decorations.pathreplacing}
\usepackage{graphicx}
\usepackage{mathrsfs}
\usepackage{quiver}
\usepackage{caption}


\renewcommand{\labelenumi}{(\theenumi)}

\usepackage{paralist}
\let\itemize\compactitem
\let\enditemize\endcompactitem
\let\enumerate\compactenum
\let\endenumerate\endcompactenum
\let\description\compactdesc
\let\enddescription\endcompactdesc

\newtheorem*{maintheorem}{Main Theorem} 

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{theorem*}{Theorem}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}[theorem]{Question}
\newtheorem{assumptions}{Assumptions}
\newtheorem*{assumptions*}{Assumptions}
\newtheorem*{assumption}{Assumption}
\newtheorem*{proposition*}{Proposition}


\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{example}[theorem]{Example} 
\newtheorem{figureexample}[theorem]{Figure} 

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}

\renewcommand{\thefigure}{\thesection.\arabic{theorem}}

\setcounter{tocdepth}{2}






